Guaranteeing Safety for Neural Network-Based Aircraft Collision Avoidance Systems

The decision logic for the ACAS X family of aircraft collision avoidance systems is represented as a large numeric table. Due to storage constraints of certified avionics hardware, neural networks have been suggested as a way to significantly compress the data while still preserving performance in terms of safety. However, neural networks are complex continuous functions with outputs that are difficult to predict. Because simulations evaluate only a finite number of encounters, simulations are not sufficient to guarantee that the neural network will perform correctly in all possible situations. We propose a method to provide safety guarantees when using a neural network collision avoidance system. The neural network outputs are bounded using neural network verification tools like Reluplex and Reluval, and a reachability method determines all possible ways aircraft encounters will resolve using neural network advisories and assuming bounded aircraft dynamics. Experiments with systems inspired by ACAS X show that neural networks giving either horizontal or vertical maneuvers can be proven safe. We explore how relaxing the bounds on aircraft dynamics can lead to potentially unsafe encounters and demonstrate how neural network controllers can be modified to guarantee safety through online costs or lowering alerting cost. The reachability method is flexible and can incorporate uncertainties such as pilot delay and sensor error. These results suggest a method for certifying neural network collision avoidance systems for use in real aircraft.

==> VerticalGeometryTEMP.tex <==
\begin{tikzpicture}
\node [aircraft top,fill=black,minimum width=5cm,rotate=0] (own) at (0,0) {};
\end{tikzpicture}
